TaskNorm: Rethinking Batch Normalization for Meta-Learning

Modern meta-learning approaches for image classification rely on increasingly deep networks to achieve state-of-the-art performance, making batch normalization an essential component of meta-learning pipelines. However, the hierarchical nature of the meta-learning setting presents several challenges that can render conventional batch normalization ineffective, giving rise to the need to rethink normalization in this setting. We evaluate a range of approaches to batch normalization for meta-learning scenarios, and develop a novel approach that we call TaskNorm. Experiments on fourteen datasets demonstrate that the choice of batch normalization has a dramatic effect on both classification accuracy and training time for both gradient based and gradient-free meta-learning approaches. Importantly, TaskNorm is found to consistently improve performance. Finally, we provide a set of best practices for normalization that will allow fair comparison of meta-learning algorithms.

==> tables/normalization_methods.tex <==
\begin{table*}[t]
\caption{Summary of the moment calculations for various normalization methods.\todosn{Use LaTeX's resizebox or adjustbox commands here to make the table exactly fit the page width, see e.g. \url{https://tex.stackexchange.com/questions/163246/resize-a-tabular-object-to-textwidth}.
Also add horizontal lines spanning two columns each under Meta-Train and Meta-Test headings to make it clear that each covers the exact two columns below it.  The abbreviations used for the normalization methods are not all clear (CBN,TBN,LN,IN) without reading Section 3.1; maybe consider adding the citations or at least the full name here?}}
\todojb{The plan is to replace this table (which is tricky to parse) with small computation diagrams that we are still working on, but we should have in place this week.}
%
\label{tab:normalization_methods}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l c c c c}
\toprule
Normalization & \multicolumn{2}{c}{Meta-Train}                                                                                & \multicolumn{2}{c}{Meta-Test} \\
Method        & Context                                               & Target                                                & Context                 & Target \\
\midrule
CBN           & $\vmu_{BN}(D^\tau)$, $\vsigma_{BN}^2(D^\tau)$         & $\vmu_{BN}(T^\tau)$, $\vsigma_{BN}^2(T^\tau)$         & $\vmu_r$, $\vsigma_r^2$                               & $\vmu_r$, $\vsigma_r^2$ \\
TBN           & $\vmu_{BN}(D^\tau)$, $\vsigma_{BN}^2(D^\tau)$         & $\vmu_{BN}(T^\tau)$, $\vsigma_{BN}^2(T^\tau)$         & $\vmu_{BN}(D^\tau)$, $\vsigma_{BN}^2(D^\tau)$         & $\vmu_{BN}(T^\tau)$, $\vsigma_{BN}^2(T^\tau)$ \\
LN            & $\vmu_{LN}(\vx)$, $\vsigma_{LN}^2(\vx)$               & $\vmu_{LN}(\vx)$, $\vsigma_{LN}^2(\vx)$               & $\vmu_{LN}(\vx)$, $\vsigma_{LN}^2(\vx)$               & $\vmu_{LN}(\vx)$, $\vsigma_{LN}^2(\vx)$ \\
IN            & $\vmu_{IN}(\vx)$, $\vsigma_{IN}^2(\vx)$               & $\vmu_{IN}(\vx)$, $\vsigma_{IN}^2(\vx)$               & $\vmu_{IN}(\vx)$, $\vsigma_{IN}^2(\vx)$               & $\vmu_{IN}(\vx)$, $\vsigma_{IN}^2(\vx)$ \\
Meta-BN       & $\vmu_{BN}(D^\tau)$, $\vsigma_{BN}^2(D^\tau)$         & $\vmu_{BN}(D^\tau)$, $\vsigma_{BN}^2(D^\tau)$         & $\vmu_{BN}(D^\tau)$, $\vsigma_{BN}^2(D^\tau)$         & $\vmu_{BN}(D^\tau)$, $\vsigma_{BN}^2(D^\tau)$ \\
\tasknorm{}   & $\vmu_{TN}(\vx, D^\tau)$, $\vsigma_{TN}(\vx, D^\tau)$ & $\vmu_{TN}(\vx, D^\tau)$, $\vsigma_{TN}(\vx, D^\tau)$ & $\vmu_{TN}(\vx, D^\tau)$, $\vsigma_{TN}(\vx, D^\tau)$ & $\vmu_{TN}(\vx, D^\tau)$, $\vsigma_{TN}(\vx, D^\tau)$ \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{small}
\end{center}
\end{table*}
